Rethinking Localization Map: Towards Accurate Object Perception with Self-Enhancement Maps

Recently, remarkable progress has been made in weakly supervised object localization (WSOL) to promote object localization maps. The common practice of evaluating these maps applies an indirect and coarse way, i.e., obtaining tight bounding boxes which can cover high-activation regions and calculating intersection-over-union (IoU) scores between the predicted and ground-truth boxes. This measurement can evaluate the ability of localization maps to some extent, but we argue that the maps should be measured directly and delicately, i.e., comparing the maps with the ground-truth object masks pixel-wisely. To fulfill the direct evaluation, we annotate pixel-level object masks on the ILSVRC validation set. We propose to use IoU-Threshold curves for evaluating the real quality of localization maps. Beyond the amended evaluation metric and annotated object masks, this work also introduces a novel self-enhancement method to harvest accurate object localization maps and object boundaries with only category labels as supervision. We propose a two-stage approach to generate the localization maps by simply comparing the similarity of point-wise features between the high-activation and the rest pixels. Based on the predicted localization maps, we explore to estimate object boundaries on a very large dataset. A hard-negative suppression loss is proposed for obtaining fine boundaries. We conduct extensive experiments on the ILSVRC and CUB benchmarks. In particular, the proposed Self-Enhancement Maps achieve the state-of-the-art localization accuracy of 54.88% on ILSVRC. The code and the annotated masks are released at https://github.com/xiaomengyc/SEM.

==> body/tables/comp_cub_methods.tex <==
\begin{table}[t]\setlength{\tabcolsep}{8pt}
  \centering
  \small
  \begin{tabular}{lcccc}
     \toprule[0.2em]
     Method & SHM & AP & IoU & Peak-T\\
     \toprule[0.2em]
     \multirow{2}{*}{CAM~\cite{zhou2015cnnlocalization} }
     & w/o  & 68.1  &  47.06 & 37\\
     & w/ & \textbf{75.63} & \textbf{48.59} & 171\\
     \hline
     \multirow{2}{*}{HaS~\cite{singh2017hide} }
     & w/o  & 52.80  & 56 \\
     & w/ & \textbf{} & \textbf{} \\
     \hline
     \multirow{2}{*}{ACoL~\cite{zhang2018adversarial}}
     & w/o  &  &  \\
     & w/ & \textbf{} & \textbf{} \\
     \hline
     \multirow{2}{*}{CutMix~\cite{yun2019cutmix}}
     & w/o &  &  \\
     & w/ & \textbf{} & \textbf{} \\
     \hline
     \multirow{2}{*}{SPG~\cite{zhang2018self}}
     & w/o &   &  \\
     & w/ & \textbf{} & \textbf{} \\
     \hline
     \multirow{2}{*}{ADL~\cite{Choe_2019_CVPR}}
     & w/o &   &  & \\
     & w/ & \textbf{} & \textbf{} \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on CUB calculated with the object masks.}
  \label{tab:comp-cub-nets-sal}
  \vspace{-15pt}
\end{table}

==> body/tables/comp_ilsvrc_err.tex <==
% \begin{table*}[t]\setlength{\tabcolsep}{15pt}
\begin{table}[t]\setlength{\tabcolsep}{5pt}
  \centering
  \footnotesize
%   \small
%   \tiny
  \begin{tabular}{llccccc}
     \toprule[0.2em]
    %  \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Localization Error} & Classification Error\\
     \multirow{2}{*}{Backbone} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Loc. Err.} & Cls. Err.\\
    %  methods & backbone & \multicolumn{3}{c}{localization err.} \\
    %  \cline{3-5}
      & & Top-1  & Gt-known & Top-1 \\
    % \hline
    %  GoogLeNet & CAM~\cite{zhou2015cnnlocalization} & GoogLeNet & 56.40  & 41.34 & 31.9 \\
    %  HaS-32~\cite{singh2017hide} &GoogLeNet& 54.53 & 39.43 & 32.5 \\
    %  ACoL~\cite{zhang2018adversarial} & GoogLeNet & 53.28  & -  & 29.0 \\
     \toprule[0.2em]
     \multirow{6}{*}{VGG16~\cite{simonyan2014very}}
    %  & Backprop~\cite{simonyan2013deep}  & 61.12 & - \\
    %  & CAM~\cite{zhou2015cnnlocalization}  & 57.20 & - &  31.2 \\
     & {$\dagger$}CAM~\cite{zhou2015cnnlocalization}  & 54.85 & 39.94 &  28.8 \\
     &   & 57.20~\cite{zhou2015cnnlocalization} & - &  31.2~\cite{zhou2015cnnlocalization} \\
    %  & HaS~\cite{singh2017hide} & & & \\
     & ADL~\cite{Choe_2019_CVPR} & 55.08 & - & 32.2  \\
     & ACoL~\cite{zhang2018adversarial}  & 54.17 & 37.04 & 32.5 \\
     & DFM~\cite{zhou2019dual} & 52.59 & - & 31.4 \\
     & SHM~\textsubscript{CAM} & \textbf{52.47} & \textbf{36.53} & 28.8 \\
    %  \hline
    %  InceptionV3~\cite{szegedy2016rethinking} & {$^\dagger$}CAM~\cite{zhou2015cnnlocalization} &  53.71 & 37.32 & 26.7 \\
    %  & SPG~\cite{zhang2018self}  & 51.40  & 35.31 & 30.3 \\
    %  & ADL~\cite{Choe_2019_CVPR}  & 51.29 & - & 27.2 \\
    %  & SCM & \textbf{46.96} & \textbf{30.96} & 26.7\\
     \hline
     \multirow{3}{*}{ResNet50~\cite{he2016deep}}
    %  & CAM~\cite{zhou2015cnnlocalization}  &   54.65 & - & 23.94 \\
     & {$\dagger$}CAM~\cite{zhou2015cnnlocalization}  &   48.87 & 37.29 & 24.9 \\
    %  &   &   54.65~\cite{zhou2019dual} & - & 23.94~\cite{zhou2019dual} \\
     & DFM~\cite{zhou2019dual} & 50.29 & - & 22.2 \\
     & SHM~\textsubscript{CAM} & \textbf{46.16} & \textbf{33.00} & 24.9 \\
     \hline
     \multirow{3}{*}{ResNet101~\cite{he2016deep}}
    %  & CAM~\cite{zhou2015cnnlocalization}  & 53.84 & - & 23.07    \\
     & {$\dagger$}CAM~\cite{zhou2015cnnlocalization}  & 47.06 & 35.87 & 20.9    \\
    %  &   & 53.84~\cite{zhou2015cnnlocalization} & - & 23.07~\cite{zhou2015cnnlocalization}    \\
     & DFM~\cite{zhou2019dual} & 49.35 & - & 22.8 \\
     & SHM~\textsubscript{CAM} &  \textbf{45.12} & \textbf{32.85} & 20.9\\
    %  \hline
    %  ResNet50-SE & CAM~\cite{zhou2015cnnlocalization}  &   & & 21.1  \\
    %  & ADL~\cite{Choe_2019_CVPR} & 51.47 & - & 24.15\\
    %  & Ours & & & 21.1\\
     \hline
     \multirow{8}{*}{InceptionV3~\cite{szegedy2016rethinking}}
     & {$\dagger$}CAM~\cite{zhou2015cnnlocalization} &  53.71 & 37.32 & 26.7 \\
     & SPG~\cite{zhang2018self}  & 51.40  & 35.31 & 30.3 \\
     & ADL~\cite{Choe_2019_CVPR}  & 51.29 & - & 27.2 \\
     & {$\dagger$}HaS & 49.59 & 33.60 & 28.3\\
     & {$\dagger$}CutMix & 51.37 & 35.00 & 30.2\\
     & SEM~\textsubscript{HaS} & 48.41 & 31.62 & 28.3\\
     & SEM~\textsubscript{CutMix} & 49.21 & 31.02 & 30.2\\
     & SEM~\textsubscript{CAM} & \textbf{46.96} & \textbf{30.96} & 26.7\\
    %  & SHM~\textsubscript{SPG} &  &  & \\
     \toprule[0.1em]
  \end{tabular}
  \caption{Localization error of the inferred bounding boxes on the ILSVRC validation set. {$\dagger$}: The results of our re-implemented model.
  }\label{tab-comp-ilsvrc}
\end{table}



==> body/tables/comp_methods_test.tex <==
\begin{table}[t]\setlength{\tabcolsep}{12pt}
  \centering
  \small
  \begin{tabular}{lclcc}
     \toprule[0.2em]
    Method & SEM & AP & IoU & Peak-T\\
     \toprule[0.2em]
     \multirow{2}{*}{CAM~\cite{zhou2015cnnlocalization}}
     & w/o & 71.06 & 50.13 & 38 \\
     & w/ & 72.54 & 55.67 & 93 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{HaS~\cite{singh2017hide}}
    %   & w/o &   & 42.69 & 112 \\
      & w/o & 71.07  & 51.44 & 38 \\
      & w/ & 72.24  & 55.15 & 108 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{ACoL~\cite{zhang2018adversarial}}
      & w/o  & 68.64  & 51.90 & 65 \\
    %   & w/o  &   & 43.84 & 54 \\
      & w/  &  67.92 & 52.80 & 115 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{CutMix~\cite{yun2019cutmix}}
     & w/o  & 70.45  & 50.97 & 34 \\
     & w/  & 71.78  & 55.28 & 101 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{SPG~\cite{zhang2018self}}
     & w/o  & 71.53 & 51.76 & 37  \\
     & w/  &  72.59 & 56.92 & 139  \\
     \bottomrule[0.1em]
     \multirow{2}{*}{ADL~\cite{Choe_2019_CVPR}}
     & w/o  & 70.19  & 49.96 & 42  \\
     & w/  & 67.26  & 50.98 & 144  \\
    %  DANet  &   &  &  \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on ILSVRC calculated with the object masks on the test set. \todoblue{add peak threshold}
  }\label{tab:comp-nets-sal}
\end{table}

% \begin{table}[t]\setlength{\tabcolsep}{12pt}
%   \centering
%   \small
%   \begin{tabular}{llcc}
%      \toprule[0.2em]
%     Method & AP & IoU & Peak-T\\
%      \toprule[0.2em]
%      CAM  &   & 50.13 & 38 \\
%      HaS  &   & 42.69 & 112 \\
%      ACoL  &   & 43.84 & 54 \\
%      SPG  &   & 51.76 & 37  \\
%      ADL  &   & 49.96 & 42 \\
%     %  DANet  &   &  &  \\
%      \bottomrule[0.1em]
%      CAM+SEM  &  63.30 & 45.13 &  \\
%      SPG+SEM  &  63.30 & 45.13 &  \\
%      ADL+SEM  &  63.30 & 45.13 &  \\
%      DANet+SEM  &  63.30 & 45.13 &  \\
%      \bottomrule[0.1em]
%   \end{tabular}
%   \caption{Localization AP and IoU on ILSVRC calculated with the object masks on the test set. \todoblue{add peak threshold}
%   }\label{tab:comp-nets-sal}
% \end{table}


==> body/tables/comp_methods_val.tex <==
\begin{table}[t]\setlength{\tabcolsep}{12pt}
  \centering
  \small
  \begin{tabular}{lclcc}
     \toprule[0.2em]
    Method & SEM & AP & IoU & Peak-T\\
     \toprule[0.2em]
     \multirow{2}{*}{CAM~\cite{zhou2015cnnlocalization}}
     & w/o & 70.68 & 50.58 & 33 \\
     & w/ & 72.78 & 55.95 & 93 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{HaS~\cite{singh2017hide}}
    %   & w/o &   & 42.87 & 114 \\
      & w/o & 70.79  & 51.20 & 37 \\
      & w/ & 72.46  & 55.43 & 109 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{ACoL~\cite{zhang2018adversarial}}
    %   & w/o  &   & 43.77 & 54 \\
      & w/o  & 68.15 & 51.59 & 62 \\
      & w/  & 67.89  & 72.74 & 115 \\
     \bottomrule[0.1em]
     \multirow{2}{*}{CutMix~\cite{yun2019cutmix}}
     & w/o  & 70.78  & 50.89 & 34  \\
     & w/  & 72.12  & 55.59 & 101  \\
     \bottomrule[0.1em]
     \multirow{2}{*}{SPG~\cite{zhang2018self}}
     & w/o  & 71.18  & 51.28 & 36  \\
     & w/  & 72.77  & 57.02 & 139  \\
     \bottomrule[0.1em]
     \multirow{2}{*}{ADL~\cite{Choe_2019_CVPR}}
     & w/o  & 69.89  & 50.01 & 42  \\
     & w/  & 67.32  & 51.10 & 144  \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on ILSVRC calculated with the object masks on the val set. \todoblue{add peak threshold}
  }\label{tab:comp-nets-sal}
\end{table}


==> body/tables/comp_nets_sal.tex <==
\begin{table}[t]\setlength{\tabcolsep}{12pt}
  \centering
  \small
  \begin{tabular}{llcc}
     \toprule[0.2em]
     Backbone & Method & AP & IoU\\
     \toprule[0.2em]
     \multirow{2}{*}{VGG16~\cite{simonyan2014very}}
     & CAM~\cite{zhou2015cnnlocalization}  &  62.23 & 44.38 \\
    %  & HaS~\cite{singh2017hide}  & 57.85  \\
    %  & ACoL~\cite{zhang2018adversarial}  &  59.64  & 43.05\\
     & SCM & \textbf{65.14} & \textbf{46.68}\\
     \hline
     \multirow{2}{*}{ResNet50~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  &  63.02 & 45.63 \\
     & SCM & \textbf{67.43} & \textbf{51.38} \\
     \hline
     \multirow{2}{*}{ResNet101~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  & 65.29 & 47.32 \\
     & SCM & \textbf{68.32} & \textbf{52.03} \\
     \hline
     \multirow{2}{*}{InceptionV3~\cite{szegedy2016rethinking}}
     & CAM~\cite{zhou2015cnnlocalization} &  69.09 & 49.58 \\
    %  & SPG~\cite{zhang2018self}  &  66.68 & 49.10\\
     & SCM & \textbf{72.02} & \textbf{54.89} \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on ILSVRC calculated with the object masks.}\label{tab:comp-nets-sal}
  \vspace{-15pt}
\end{table}


==> body/tables/comp_nets_sal_test.tex <==
\begin{table}[t]\setlength{\tabcolsep}{12pt}
  \centering
  \small
  \begin{tabular}{llcc}
     \toprule[0.2em]
     Backbone & Method & AP & IoU\\
     \toprule[0.2em]
     \multirow{2}{*}{VGG16~\cite{simonyan2014very}}
     & CAM~\cite{zhou2015cnnlocalization}  &  62.82 & 44.89 \\
     & SCM & \textbf{65.14} & \textbf{47.53}\\
     \hline
     \multirow{2}{*}{ResNet50~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  &  64.51 & 45.98 \\
     & SCM & \textbf{67.83} & \textbf{52.01} \\
     \hline
     \multirow{2}{*}{ResNet101~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  & 66.99 & 47.91 \\
     & SCM & \textbf{68.87} & \textbf{52.84} \\
     \hline
     \multirow{2}{*}{InceptionV3~\cite{szegedy2016rethinking}}
     & CAM~\cite{zhou2015cnnlocalization} &  71.06 & 51.17 \\
     & SCM & \textbf{72.54} & \textbf{55.67} \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on ILSVRC calculated with the object masks on the test set.}\label{tab:comp-nets-sal}
\end{table}

==> body/tables/comp_nets_sal_val.tex <==
\begin{table}[t]\setlength{\tabcolsep}{12pt}
  \centering
  \small
  \begin{tabular}{llcc}
     \toprule[0.2em]
     Backbone & Method & AP & IoU\\
     \toprule[0.2em]
     \multirow{2}{*}{VGG16~\cite{simonyan2014very}}
     & CAM~\cite{zhou2015cnnlocalization}  &  63.30 & 45.13 \\
     & SCM & \textbf{65.03} & \textbf{47.32}\\
     \hline
     \multirow{2}{*}{ResNet50~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  &  65.18 & 46.14 \\
     & SCM & \textbf{68.12} & \textbf{52.22} \\
     \hline
     \multirow{2}{*}{ResNet101~\cite{he2016deep}}
     & CAM~\cite{zhou2015cnnlocalization}  & 67.56 & 48.16 \\
     & SCM & \textbf{69.08} & \textbf{52.91} \\
     \hline
     \multirow{2}{*}{InceptionV3~\cite{szegedy2016rethinking}}
     & CAM~\cite{zhou2015cnnlocalization} & 70.68 & 51.00 \\
     & SCM & \textbf{72.78} & \textbf{55.95} \\
     \bottomrule[0.1em]
  \end{tabular}
  \caption{Localization AP and IoU on ILSVRC calculated with the object masks on the validation set. \todoblue{add peak threshold}
  }\label{tab:comp-nets-sal}
\end{table}


==> body/tables/inception_backbone.tex <==
\begin{table}[b]\setlength{\tabcolsep}{8pt}
  \centering
  \small
  \scalebox{0.93}{
  \begin{tabular}{lccc}
    \toprule[0.2em]
      & Type & Kernel & Input Size \\
    \toprule[0.2em]
    \multirow{4}{*}{Block 1}
      & Convolution &  $3 \times 3/2$ & $3\times 320\times 320$ \\
      & Convolution &  $3 \times 3/1$ & $32\times 160\times 160$ \\
      & Convolution &  $3 \times 3/1$ & $32\times 160\times 160$ \\
      & Max Pool & $3 \times 3/2$ & $64\times 160\times 160$ \\
    \hline
    \multirow{3}{*}{Block 2}
      & Convolution &  $1 \times 1/1$ & $64\times 80\times 80$ \\
      & Convolution &  $3 \times 3/1$ & $80\times 80\times 80$ \\
      & Max Pool & $3 \times 3/2$ & $192\times 80\times 80$ \\
    \hline
    \multirow{2}{*}{Block 3}
      & 3 $\times$ Inception & Module A~\ref{fig:module_a} & $192\times 40\times 40$ \\
      & 1 $\times$ Inception & Module B~\ref{fig:module_b} & $256\times 40\times 40$ \\
    \hline
    Block 4 
      & 4 $\times$ Inception & Module C~\ref{fig:module_c} &  $288\times 40\times 40$ \\
    \hline
    \multirow{3}{*}{Block 5} 
      & Convolution &  $3 \times 3/1$ & $768\times 40\times 40$ \\
      & Convolution &  $3 \times 3/1$ & $1024\times 40\times 40$ \\
      & Convolution &  $1 \times 1/1$ & $1024\times 40\times 40$ \\
    \toprule[0.1em]
  \end{tabular}
  }
  \caption{
  Details of the InceptionV3 network following SPG~\cite{zhang2018self}. 
  The Inception modules are depicted in Figure~\ref{fig-module}.
  }\label{tab:backbone} 
  \vspace{-15pt}
\end{table}

==> body/tables/scm_algorithm.tex <==
% \begin{algorithm*}
% \lstset{caption={PyTorch}}
% \begin{lstlisting}[language=Python,frame=single]
% def get_scm_maps(M, F, K, c):
%     W, H = M.shape[-2:]
%     cam = M[c,:,:]
%     cam=(cam-cam.min())/(cam.max() - cam.min())
% \end{lstlisting}
\IncMargin{2em}
\begin{algorithm*}[htbp]
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Return}{Return}
\SetKwData{Left}{left}
\SetKwComment{tcpython}{\#}{}

\SetAlgoLined

% \Input{$M\in \mathbb{R}^{Y\times W \times H}$, $F\in \mathbb{R}^{C\times W \times H}$, $K$, $y$}
\Input{$M$, $F$, $K$, $y$}
\tcpython{\textcolor{gray}{\emph{M is top-layer feature maps of size (Y,W,H)}}}
\tcpython{\textcolor{gray}{\emph{F is high-level feature maps of size (C,W,H)}}}
\tcpython{\textcolor{gray}{\emph{K is the seed number, and y is the category label}}}

\LinesNumbered
\Output{$cam\in [0,1]^{W \times H}$, $sem \in [0,1]^{W \times H}$}
\BlankLine
\Indp c, w, h = F.shape \tcpython{\textcolor{gray}{\emph{Get the channel number and size of the input feature maps}}}


\tcpython{\textcolor{black}{Stage One}}
cam = M[y, :, :] \tcpython{\textcolor{gray}{\emph{Get the localization map of class y}}}

cam=(cam - cam.min()) / (cam.max() - cam.min()) \tcpython{\textcolor{gray}{\emph{Normalize cam maps to [0,1]}}}

\tcpython{\textcolor{black}{Stage Two}}
\_,~topk\_indices = torch.topk(cam.view(-1), K, largest=True) 
\tcpython{\textcolor{gray}{\emph{Get the indices of the seed pixels with top K scores}}}

F\_seeds = F.view(c, -1)[:, topk\_indices] \tcpython{\textcolor{gray}{\emph{Get the feature vectors of the K seeds}}}

simi = torch.nn.functional.cosine\_similarity(F.view(c, -1, 1), F\_seeds.view(c, 1, -1), dim=0) \tcpython{\textcolor{gray}{\emph{Compute the cosine similarity between F and F\_{seeds}}}}

sem,~\_ = simi.max(dim=1) \tcpython{\textcolor{gray}{\emph{Get the highest scores across the K values at each pixel}}}

sem = sem.view(w, h) \tcpython{\textcolor{gray}{\emph{Reshape to the size of (w, h)}}}

sem=(sem - sem.min()) / (sem.max() - sem.min()) \tcpython{\textcolor{gray}{\emph{Normalize sem maps to [0,1]}}}


\caption{Generating SEM localization maps in PyTorch}
\label{alg-scm}

% \vspace{-20pt}
\end{algorithm*}
\DecMargin{1em}

